Fermi Acceleration in anti-integrable limits of the standard map

We consider a dynamical system on the semi-infinite cylinder which models the high energy dynamics of a family of mechanical models. We provide conditions under which we ensure that the set of orbits undergoing Fermi acceleration has measure zero.

==> definitions.p.tex <==
% multiple inclusion guard
\makeatletter\@ifundefined{DEFINITIONS}{
\makeatletter\def\DEFINITIONS{}
%%

%Macros for critical sets, reference sections and cones
\newcommand{\tg}[1]{\textbf{T}_{#1}}
\newcommand{\phspace}{\mathbb{A}}
\newcommand{\bundle}{\mathscr{F}}
\newcommand{\criticalinternal}{C}
\newcommand{\critical}[1]{\mathbf{\criticalinternal}_{#1}}
\newcommand{\corecritical}[1]{\bar{\mathbf{\criticalinternal}}_{#1}}
\newcommand{\hcritical}[1]{\hat{\mathbf{\criticalinternal}}_{#1}}
\newcommand{\vcritical}[1]{\check{\mathbf{\criticalinternal}}_{#1}}

\newcommand{\subsetsim}{\underset{\widetilde{}}{\subset}}
\newcommand{\supsetsim}{\underset{\widetilde{}}{\supset}}

\newcommand{\slopeinternal}{h}
\newcommand{\slope}[1]{\slopeinternal_{#1}}
\newcommand{\tslope}[1]{\tilde{\slopeinternal}_{#1}}
\newcommand{\dslope}[1]{\dot{\slopeinternal}_{#1}}
\newcommand{\minslope}{\underline{\slopeinternal}}


\newcommand{\rc}{\psi_1}

\newcommand{\rr}[1]{r_{#1}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\lpm}{\mathscr{L}^\pm}

\newcommand{\escaping}{\mathscr{E}}
\newcommand{\cone}[1]{\mathcal{C}_{#1}}
%\newcommand{\const}{\mbox{Const}\cdot}
\newcommand{\Lip}{\textrm{Lip}}

%%%% Coordinate commands
\newcommand{\ct}[1]{x_{#1}}
\newcommand{\cv}[1]{y_{#1}}
\newcommand{\bcv}[1]{\bar{y}_{#1}}
\newcommand{\coo}[1]{\ct{#1},\cv{#1}}
\newcommand{\coop}[1]{\ct{#1}',\cv{#1}'}
\newcommand{\T}{Y}
\newcommand{\iT}{\T^{-1}}
\newcommand{\coof}{x,y,\rr{},\slope{},\dslope{}}
\newcommand{\V}{\hat{y}}
%Macros for the Riemann Lemma
\newcommand{\indexset}{\mathcal{J}}
\newcommand{\rslc}{a}
\newcommand{\RiemFunc}{f}

%Macros for the Equidistribution lemma
\newcommand{\bs}{E}
\newcommand{\ball}{\mathcal{B}}
\newcommand{\Tr}{\textrm{Tr}}
\newcommand{\continuous}[2]{\mathscr{C}^{#1}(#2)}
\newcommand{\expectation}{\mathbb{E}}

\newcommand{\std}{\textrm{std}}
\renewcommand{\sb}{\textrm{sb}}
\newcommand{\inva}{\textrm{inva}}
\newcommand{\aset}{\mathcal{A}}

\newtheorem*{lemmaInvPrime}{Lemma \ref{l_invariance}$'$}

}{} %%\@ifundefined{DEFINITIONS}

